A Flexible Stochastic Conditional Duration Model

We introduce a new stochastic duration model for transaction times in asset markets. We argue that widely accepted rules for aggregating seemingly related trades mislead inference pertaining to durations between unrelated trades: while any two trades executed in the same second are probably related, it is extremely unlikely that all such pairs of trades are, in a typical sample. By placing uncertainty about which trades are related within our model, we improve inference for the distribution of durations between unrelated trades, especially near zero. We introduce a normalized conditional distribution for durations between unrelated trades that is both flexible and amenable to shrinkage towards an exponential distribution, which we argue is an appropriate first-order model. Thanks to highly efficient draws of state variables, numerical efficiency of posterior simulation is much higher than in previous studies. In an empirical application, we find that the conditional hazard function for durations between unrelated trades varies much less than what most studies find. We claim that this is because we avoid statistical artifacts that arise from deterministic trade-aggregation rules and unsuitable parametric distributions.

==> results-diurnal-all-pot.tex <==
          $\delta_1$ &  2.056 & 1.28e-01 & 0.880 &  2.055 & 1.30e-01 & 0.745 &  2.054 & 1.30e-01 & 0.738 &  2.056 & 1.30e-01 & 0.758 \\
          $\delta_2$ &  2.207 & 1.03e-01 & 0.955 &  2.205 & 1.05e-01 & 0.855 &  2.205 & 1.05e-01 & 0.825 &  2.207 & 1.04e-01 & 0.763 \\
          $\delta_3$ &  2.356 & 8.92e-02 & 0.990 &  2.353 & 9.17e-02 & 0.906 &  2.354 & 9.20e-02 & 0.857 &  2.354 & 9.11e-02 & 0.868 \\
          $\delta_4$ &  2.574 & 8.24e-02 & 0.965 &  2.567 & 8.41e-02 & 0.926 &  2.568 & 8.48e-02 & 0.835 &  2.569 & 8.40e-02 & 0.885 \\
          $\delta_5$ &  2.781 & 8.30e-02 & 0.936 &  2.769 & 8.48e-02 & 1.013 &  2.771 & 8.45e-02 & 0.832 &  2.771 & 8.49e-02 & 0.799 \\
          $\delta_6$ &  2.870 & 8.21e-02 & 0.979 &  2.862 & 8.38e-02 & 1.054 &  2.864 & 8.41e-02 & 0.862 &  2.863 & 8.42e-02 & 0.864 \\
          $\delta_7$ &  2.917 & 8.23e-02 & 1.141 &  2.912 & 8.42e-02 & 0.986 &  2.913 & 8.36e-02 & 0.780 &  2.913 & 8.35e-02 & 0.948 \\
          $\delta_8$ &  3.014 & 8.23e-02 & 1.114 &  3.007 & 8.48e-02 & 0.936 &  3.008 & 8.48e-02 & 0.848 &  3.008 & 8.45e-02 & 0.887 \\
          $\delta_9$ &  3.091 & 8.36e-02 & 0.876 &  3.079 & 8.61e-02 & 0.802 &  3.080 & 8.60e-02 & 0.922 &  3.079 & 8.56e-02 & 0.916 \\
       $\delta_{10}$ &  3.048 & 8.31e-02 & 0.957 &  3.034 & 8.56e-02 & 0.788 &  3.035 & 8.52e-02 & 0.842 &  3.035 & 8.44e-02 & 0.723 \\
       $\delta_{11}$ &  2.918 & 8.24e-02 & 1.033 &  2.908 & 8.39e-02 & 0.764 &  2.909 & 8.43e-02 & 0.881 &  2.909 & 8.36e-02 & 0.813 \\
       $\delta_{12}$ &  2.833 & 8.20e-02 & 0.967 &  2.821 & 8.44e-02 & 0.913 &  2.821 & 8.36e-02 & 0.853 &  2.821 & 8.36e-02 & 0.907 \\
       $\delta_{13}$ &  2.739 & 8.33e-02 & 0.922 &  2.722 & 8.58e-02 & 0.827 &  2.722 & 8.60e-02 & 0.930 &  2.722 & 8.52e-02 & 0.793 \\
       $\delta_{14}$ &  2.518 & 8.85e-02 & 0.922 &  2.503 & 9.15e-02 & 0.899 &  2.505 & 9.10e-02 & 0.975 &  2.504 & 9.13e-02 & 0.838 \\
       $\delta_{15}$ &  2.211 & 1.02e-01 & 0.850 &  2.203 & 1.05e-01 & 0.768 &  2.204 & 1.04e-01 & 0.900 &  2.205 & 1.04e-01 & 0.821 \\
       $\delta_{16}$ &  1.837 & 1.36e-01 & 0.719 &  1.828 & 1.39e-01 & 0.536 &  1.829 & 1.39e-01 & 0.631 &  1.831 & 1.38e-01 & 0.639 \\


==> results-diurnal-all-ry.tex <==
          $\delta_1$ &  1.625 & 1.27e-01 & 0.881 &  1.621 & 1.28e-01 & 0.798 &  1.622 & 1.28e-01 & 0.739 &  1.618 & 1.28e-01 & 0.808 \\
          $\delta_2$ &  1.817 & 1.04e-01 & 0.954 &  1.812 & 1.04e-01 & 0.873 &  1.812 & 1.04e-01 & 0.746 &  1.809 & 1.04e-01 & 0.749 \\
          $\delta_3$ &  1.927 & 9.23e-02 & 1.151 &  1.922 & 9.22e-02 & 0.886 &  1.922 & 9.16e-02 & 0.751 &  1.919 & 9.22e-02 & 0.680 \\
          $\delta_4$ &  2.090 & 8.44e-02 & 0.861 &  2.085 & 8.52e-02 & 1.104 &  2.086 & 8.49e-02 & 0.741 &  2.082 & 8.51e-02 & 0.767 \\
          $\delta_5$ &  2.254 & 8.52e-02 & 0.829 &  2.249 & 8.50e-02 & 0.936 &  2.251 & 8.49e-02 & 0.893 &  2.247 & 8.51e-02 & 0.719 \\
          $\delta_6$ &  2.286 & 8.39e-02 & 1.054 &  2.282 & 8.43e-02 & 0.947 &  2.283 & 8.44e-02 & 0.905 &  2.280 & 8.44e-02 & 0.831 \\
          $\delta_7$ &  2.361 & 8.41e-02 & 0.911 &  2.358 & 8.46e-02 & 0.770 &  2.358 & 8.39e-02 & 0.866 &  2.355 & 8.49e-02 & 0.718 \\
          $\delta_8$ &  2.463 & 8.47e-02 & 1.031 &  2.459 & 8.51e-02 & 0.927 &  2.460 & 8.46e-02 & 0.878 &  2.456 & 8.46e-02 & 0.860 \\
          $\delta_9$ &  2.560 & 8.63e-02 & 0.750 &  2.555 & 8.69e-02 & 0.759 &  2.556 & 8.61e-02 & 0.918 &  2.552 & 8.57e-02 & 0.899 \\
       $\delta_{10}$ &  2.548 & 8.60e-02 & 0.807 &  2.543 & 8.64e-02 & 0.775 &  2.544 & 8.65e-02 & 0.849 &  2.541 & 8.64e-02 & 0.750 \\
       $\delta_{11}$ &  2.452 & 8.48e-02 & 0.928 &  2.448 & 8.52e-02 & 0.945 &  2.449 & 8.52e-02 & 0.802 &  2.446 & 8.53e-02 & 0.759 \\
       $\delta_{12}$ &  2.335 & 8.45e-02 & 0.986 &  2.331 & 8.48e-02 & 1.094 &  2.332 & 8.44e-02 & 1.036 &  2.328 & 8.53e-02 & 0.823 \\
       $\delta_{13}$ &  2.238 & 8.67e-02 & 0.954 &  2.234 & 8.69e-02 & 0.812 &  2.234 & 8.61e-02 & 0.829 &  2.231 & 8.67e-02 & 0.758 \\
       $\delta_{14}$ &  2.024 & 9.20e-02 & 0.904 &  2.020 & 9.21e-02 & 0.908 &  2.021 & 9.19e-02 & 0.838 &  2.018 & 9.27e-02 & 0.671 \\
       $\delta_{15}$ &  1.716 & 1.04e-01 & 0.997 &  1.712 & 1.05e-01 & 0.839 &  1.713 & 1.05e-01 & 0.837 &  1.710 & 1.05e-01 & 0.795 \\
       $\delta_{16}$ &  1.288 & 1.37e-01 & 0.706 &  1.282 & 1.38e-01 & 0.604 &  1.284 & 1.37e-01 & 0.580 &  1.281 & 1.38e-01 & 0.594 \\


==> results-diurnal-reg-pot.tex <==
          $\delta_1$ &  2.039 & 1.23e-01 & 0.939 &  2.046 & 1.25e-01 & 1.038 &  2.045 & 1.24e-01 & 0.827 &  2.045 & 1.23e-01 & 0.867 \\
          $\delta_2$ &  2.190 & 9.83e-02 & 0.974 &  2.199 & 1.02e-01 & 1.170 &  2.197 & 9.99e-02 & 0.977 &  2.197 & 9.94e-02 & 0.910 \\
          $\delta_3$ &  2.340 & 8.62e-02 & 1.111 &  2.347 & 8.87e-02 & 0.863 &  2.346 & 8.76e-02 & 1.032 &  2.346 & 8.71e-02 & 0.962 \\
          $\delta_4$ &  2.558 & 7.92e-02 & 1.057 &  2.558 & 8.23e-02 & 0.983 &  2.559 & 8.05e-02 & 0.893 &  2.559 & 8.06e-02 & 0.904 \\
          $\delta_5$ &  2.766 & 7.96e-02 & 0.980 &  2.761 & 8.27e-02 & 0.994 &  2.762 & 8.20e-02 & 0.887 &  2.762 & 8.19e-02 & 0.905 \\
          $\delta_6$ &  2.851 & 7.94e-02 & 0.981 &  2.849 & 8.20e-02 & 1.012 &  2.848 & 8.13e-02 & 0.970 &  2.849 & 8.09e-02 & 1.023 \\
          $\delta_7$ &  2.898 & 7.94e-02 & 0.977 &  2.899 & 8.23e-02 & 0.980 &  2.897 & 8.09e-02 & 0.921 &  2.899 & 8.05e-02 & 1.038 \\
          $\delta_8$ &  3.004 & 7.96e-02 & 0.876 &  3.002 & 8.27e-02 & 1.046 &  3.002 & 8.14e-02 & 0.918 &  3.003 & 8.13e-02 & 0.995 \\
          $\delta_9$ &  3.085 & 8.16e-02 & 0.935 &  3.077 & 8.44e-02 & 0.875 &  3.079 & 8.31e-02 & 0.893 &  3.079 & 8.26e-02 & 0.973 \\
       $\delta_{10}$ &  3.036 & 8.07e-02 & 0.987 &  3.029 & 8.34e-02 & 0.952 &  3.030 & 8.23e-02 & 1.063 &  3.029 & 8.15e-02 & 0.909 \\
       $\delta_{11}$ &  2.900 & 7.94e-02 & 0.909 &  2.899 & 8.20e-02 & 0.867 &  2.897 & 8.11e-02 & 0.972 &  2.895 & 8.08e-02 & 0.981 \\
       $\delta_{12}$ &  2.815 & 7.98e-02 & 0.873 &  2.811 & 8.21e-02 & 1.004 &  2.809 & 8.09e-02 & 1.135 &  2.807 & 8.01e-02 & 0.851 \\
       $\delta_{13}$ &  2.734 & 8.08e-02 & 0.920 &  2.725 & 8.37e-02 & 0.959 &  2.724 & 8.16e-02 & 1.066 &  2.723 & 8.20e-02 & 1.008 \\
       $\delta_{14}$ &  2.525 & 8.64e-02 & 0.994 &  2.519 & 8.92e-02 & 0.885 &  2.519 & 8.81e-02 & 0.980 &  2.518 & 8.69e-02 & 1.017 \\
       $\delta_{15}$ &  2.225 & 9.83e-02 & 0.975 &  2.229 & 1.02e-01 & 0.827 &  2.227 & 1.00e-01 & 0.908 &  2.228 & 9.87e-02 & 0.914 \\
       $\delta_{16}$ &  1.861 & 1.30e-01 & 0.744 &  1.863 & 1.33e-01 & 0.668 &  1.864 & 1.31e-01 & 0.700 &  1.866 & 1.31e-01 & 0.821 \\


==> results-diurnal-reg-ry.tex <==
          $\delta_1$ &  1.611 & 1.20e-01 & 0.913 &  1.608 & 1.18e-01 & 1.007 &  1.606 & 1.17e-01 & 0.844 &  1.606 & 1.16e-01 & 0.852 \\
          $\delta_2$ &  1.822 & 9.71e-02 & 1.026 &  1.820 & 9.57e-02 & 1.161 &  1.819 & 9.40e-02 & 1.020 &  1.819 & 9.34e-02 & 0.982 \\
          $\delta_3$ &  1.934 & 8.62e-02 & 1.072 &  1.933 & 8.40e-02 & 0.899 &  1.930 & 8.35e-02 & 1.030 &  1.930 & 8.28e-02 & 0.965 \\
          $\delta_4$ &  2.101 & 7.92e-02 & 1.035 &  2.099 & 7.82e-02 & 0.977 &  2.097 & 7.67e-02 & 0.910 &  2.097 & 7.67e-02 & 0.899 \\
          $\delta_5$ &  2.267 & 7.93e-02 & 1.004 &  2.266 & 7.86e-02 & 1.007 &  2.266 & 7.78e-02 & 0.904 &  2.266 & 7.77e-02 & 0.958 \\
          $\delta_6$ &  2.289 & 7.89e-02 & 1.021 &  2.286 & 7.78e-02 & 0.990 &  2.286 & 7.69e-02 & 1.034 &  2.286 & 7.67e-02 & 1.022 \\
          $\delta_7$ &  2.363 & 7.90e-02 & 0.956 &  2.361 & 7.82e-02 & 0.988 &  2.357 & 7.68e-02 & 0.927 &  2.358 & 7.65e-02 & 1.048 \\
          $\delta_8$ &  2.468 & 7.91e-02 & 0.872 &  2.469 & 7.81e-02 & 1.002 &  2.464 & 7.71e-02 & 0.926 &  2.465 & 7.66e-02 & 0.997 \\
          $\delta_9$ &  2.571 & 8.12e-02 & 0.954 &  2.576 & 8.00e-02 & 0.889 &  2.572 & 7.91e-02 & 0.927 &  2.573 & 7.80e-02 & 0.953 \\
       $\delta_{10}$ &  2.557 & 8.10e-02 & 1.046 &  2.563 & 7.95e-02 & 1.005 &  2.559 & 7.85e-02 & 1.095 &  2.559 & 7.76e-02 & 0.881 \\
       $\delta_{11}$ &  2.461 & 7.93e-02 & 0.962 &  2.463 & 7.81e-02 & 0.949 &  2.462 & 7.74e-02 & 0.965 &  2.462 & 7.69e-02 & 1.001 \\
       $\delta_{12}$ &  2.349 & 7.96e-02 & 0.866 &  2.350 & 7.79e-02 & 0.995 &  2.353 & 7.69e-02 & 1.087 &  2.352 & 7.61e-02 & 0.849 \\
       $\delta_{13}$ &  2.266 & 8.11e-02 & 0.974 &  2.270 & 7.99e-02 & 0.920 &  2.273 & 7.80e-02 & 0.978 &  2.276 & 7.83e-02 & 0.989 \\
       $\delta_{14}$ &  2.064 & 8.66e-02 & 1.032 &  2.066 & 8.53e-02 & 0.852 &  2.071 & 8.43e-02 & 0.941 &  2.074 & 8.29e-02 & 0.979 \\
       $\delta_{15}$ &  1.769 & 9.73e-02 & 0.995 &  1.769 & 9.56e-02 & 0.887 &  1.775 & 9.47e-02 & 0.920 &  1.778 & 9.32e-02 & 0.892 \\
       $\delta_{16}$ &  1.362 & 1.27e-01 & 0.725 &  1.367 & 1.26e-01 & 0.694 &  1.375 & 1.23e-01 & 0.722 &  1.377 & 1.23e-01 & 0.760 \\

